Compositional Concept Generalization with Variational Quantum Circuits

Compositional generalization is a key facet of human cognition, but lacking in current AI tools such as vision-language models. Previous work examined whether a compositional tensor-based sentence semantics can overcome the challenge, but led to negative results. We conjecture that the increased training efficiency of quantum models will improve performance in these tasks. We interpret the representations of compositional tensor-based models in Hilbert spaces and train Variational Quantum Circuits to learn these representations on an image captioning task requiring compositional generalization. We used two image encoding techniques: a multi-hot encoding (MHE) on binary image vectors and an angle/amplitude encoding on image vectors taken from the vision-language model CLIP. We achieve good proof-of-concept results using noisy MHE encodings. Performance on CLIP image vectors was more mixed, but still outperformed classical compositional models.

==> Introduction.tex <==
\section{Introduction}
As humans, we are able to make sense of new situations by applying our knowledge from previously seen situations. This is called compositional generalization: having seen blue cars and red postboxes, we are able to react appropriately when we are crossing the road and a red car is speeding around the corner, even if we have never seen that particular colour of car before. In the burgeoning field of artificial intelligence and machine learning, it is desirable for systems to also have this property.

The Distributional Compositional Categorical semantic model  (DisCoCat)  introduced in \cite{Coecke2010} provides an explicitly compositional way of modelling language. It maps grammatical structure, which tells us how to compose words to form phrases and sentences, to  meanings of phrases and sentences and  encodes these in vectors and higher order tensors. The grammatical type of a word dictates the structure of the vector space it inhabits, and grammatical reductions between words are modelled as tensor contraction. 

The representation of words as vectors has been used since at least \cite{salton1975vector}. In early work, the bases of the vector space in which the words are represented is interpretable, as e.g. documents \cite{salton1975vector} or other words \cite{landauer_solution_1997}, and values of vectors at each basis are derived from the statistics of words in a given document or word co-occurrence in a corpus. 
% Later work moved to a compression of the vector space via singular value decomposition \cite{deerwester} to produce dense rather than sparse vectors. Underlying these representations is the assumption that semantic similarity is interpreted as proximity in the vector space, where proximity is usually interpreted as normalized inner product. 
For a while information theoretic  functions such as local and mutual information were used to improve on the raw word statistics. Lately, machine learning via neural networks have provided substantial advances, leading to the invention of Large Language Models. \cite{mikolov_distributed_2013} is the first in this series; it introduces  word embedding methods where the dimensions of the vector space are no longer assumed to be interpretable and the notion of semantic similarity, measured by normalized inner product, becomes the only signal used to determine the value of a vector on a given basis dimension. Semantic similarity is still, however,  determined by the co-occurrence statistics of words in a given corpus. Words are initialized with two representations: as a \emph{target word} and as a \emph{context word}. Word vectors are learnt using a \emph{contrastive learning} algorithm which increases the inner product of words that occur in the same context and which decreases the inner product of words that do not occur in the same context, approximated by drawing $K$ \emph{negative samples} randomly from the vocabulary.

Specifically, the following quantity is minimized by gradient back propagation:
\begin{equation}\label{eq:negative_sampling}
    J(\theta) = -\log \sigma(\braket{v_t|v_c}) - \sum_{k=1}^K  \log \sigma(-\braket{v_t | v_{k}})
\end{equation} 
where $\theta$ is the set of model parameters, $v_t$ is the vector of the target word, $v_c$ is the vector of the context word, $v_1, v_2, ..., v_K$ are the vector of $K$ negative samples, and $\sigma$ is the logistic learning function. This method was extended from vectors to tensors by \cite{maillard-clark-2015,wijnholds_representation_2020} to build DisCoCat-style representations.

 DisCoCat was conceived as a means of modelling linguistic meaning representations derived from the statistics of text corpora.  \cite{Lewis2023} extended it to multimodal meaning and developed methods for learning its meaning representations from labelled images. As it is explicitly compositional, we would expect the DisCoCat representations to exhibit compositional generalization. However, its representations do not straightforwardly generalize. 
 %M added
 One reason for this is that DisCoCat relies on higher order tensors and tensor contraction for modelling composition. Learning  these tensors from real data and using them in concrete computations is costly on classical computers. Tensors are however natural inhabitants of quantum systems. If modelled on quantum computers, their parameters become  easier to learnt and their computations  less costly.  DisCoCat was inspired by Categorical Quantum Mechanics \citep{abramskybob2004} and moreover has a growing ecosystem of theory and software \citep{Kartsaklis2021, Lorenz2021} enabling the implementation of DisCoCat word and sentence representations on quantum architectures such as Variational Quantum Circuits (VQCs). Using VQCs for learning meaning representations has allowed a much more efficient implementation in linguistic tasks such as text classification, question answering, and co-reference resolution \cite{mechcoecke2020quantumnatural,Meichanetzidis_2023,WazniLoPheatSadr2024}.   In this paper, we extend these methods to multimodal cognitive tasks and conjecture that the increased efficiency of quantum computing will also improve the performance of our proposed methods in the compositional generalization.

In order to test this conjecture, we use our quantum implementations on a spatial visual question answering task. We use a dataset developed by \cite{Lewis2023,pearson2024} in which the system must correctly identify the spatial relationship between objects in an image. We train meaning representations for the objects and relationships \emph{left} and \emph{right} and optimize these representations to describe the image. We find that the quantum trained representations learnt by VQCs outperform classically trained DisCoCat representations and perform on a par with modern multimodal transformer-based architectures.






\paragraph{From words to sentences to images}
The methodology suggested in \cite{Lewis2023} modelled images as word vectors.  In this paper, we also wish to model images as phrase and sentence vectors. In section \ref{sec:discocat}, we will outline a  theoretical framework for generating the multimodal phrase and sentence vectors that we will use in this paper. Again, basis dimensions in a sentence vector space are not assumed to have any particular interpretation, and one key driver of determining the values of a sentence vector is semantic similarity as measured by inner product. So, for example, we expect a sentence vector for the image wherein  `kittens drink milk' to have a higher normalized inner product with images where `black cats lap water' than with those where `three children have muddy foreheads'.

In \cite{radford_learning_2021}, the contrastive learning paradigm is extended from word-word pairs as in \eqref{eq:negative_sampling} to pairs of sentence and image vectors. The assumption underlying this method is that sentence and image vectors lie in the same semantic space, and we wish to increase the similarity of images to sentences that correctly describe those images, and decrease the similarity of image vectors to sentences that do not describe those images. For example, with one negative sample, we might have 

\begin{equation}\label{eq:contrastive_images}
    J(\theta) = -\log \sigma(\braket{{\textcolor{red}{\blacksquare}}|red\_square}) - \log\sigma(-\braket{{\textcolor{red}{\blacksquare}}|blue\_circle})
\end{equation}.

In \cite{Lewis2023}, the contrastive learning paradigm is leveraged to learn compositional word representations from the images using the DisCoCat framework, which we describe in section \ref{sec:classicalexp}. 



==> Reviews-QPL.tex <==


SUBMISSION: 97
TITLE: Compositional Concept Generalization with  Variational Quantum Circuits


----------------------- REVIEW 1 ---------------------
SUBMISSION: 97
TITLE: Compositional Concept Generalization with  Variational Quantum Circuits
AUTHORS: Hala Hawashin, Beth Pearson, Martha Lewis and Mehrnoosh Sadrzadeh

----------- Overall evaluation -----------
SCORE: -1 (weak reject)
----- TEXT:
[copy-paste into a markdown reader for formatting]


This paper studies compositional generalisation for multimodal (text and image) models in the DisCoCat family.

## SUMMARY (as I understood the paper)
### Task
The dataset consists of a selection of images containing two objects, each paired with two candidate captions the model must chose between. The (correct) captions are of the form
  (0) 'ShapeX is left/right of shapeY',
while the distractors look like:
  (1) 'ShapeX is right/left of shapeY' (incorrect direction) or
  (2) 'ShapeY is left/right of shapeX' (wrong noun order),
depending on the task.

Two sub-tasks are derived from this dataset.
  (1) [Preposition-RL] can the model distinguish between the prepositions 'isLeftOf' and 'isRightOf'.
  (2) [Noun-Swap] Given that isLeftOf is fixed to be isRightOf with its inputs swapped around, does the model learn an asymmetric embedding for isLeftOf (equiv. isRightOf).

### Dataset splits
The data is split into a train set, in-distribution (ID) and out-of-distribution (OOD) valid and test sets, in which the OOD label combinations do not feature in the train set. This is a test of compositional generalisation since the OOD sets are systematic recombinations of the labels seen in training that do not themselves feature in the training set.

### DisCoCat
These models employ a custom simplified grammar based on the usual pregroups, with vocabulary consisting of the different shape nouns, and transitive verbs capturing the prepositional phrases 'isLeftOf' and 'isRightOf'. They are interpreted with either direct vector semantics ('classical-DisCoCat'), or as quantum circuits via some rewrites and ansatze.

### Model
Goal: given an image, and its associated embedding, learn caption word embeddings such that the correct caption has a larger overlap with the image than the incorrect caption.

Various methods are compared:
Classic-CLIP (frozen): pre-trained image and text embedding pair (512 dimensions for images, also 512? for sentences?).
Classic-CLIP (fine-tuned): fine-tuned version of CLIP on the given dataset.

Quantum-CLIP: image embedding obtained by converting the classical CLIP embedding into a quantum state via amplitude encoding after reducing the dimension to 36 via PCA (=> 6 qubits?). Text embedding is DisCoCat style with a 3 leg tensor for the prepositions.
Quantum-OHE: the image embeddings are constructed manually, using 9 qubits total. Text embedding is DisCoCat style with a 3 leg tensor for the prepositions.

Each of the quantum embeddings are trained with both IQP and Sim14 ansatze. There is no mention of the dimension of the quantum n or s types, but the figures suggest they are both 1 qubit each.

Classical-discocat: discocat style embedding using the copy-subject spider decomposition for  transitive verbs. s ‎= n = image = 786 dimensions

### Methods
Word embeddings are trained using contrastive learning with respect to the images. This involves optimising the difference between the overlap of the correct caption, and the sum of overlaps of the incorrect captions.

****For classical-discocat there are 4 incorrect captions. The dataset suggests the other models have access to just one incorrect caption (?)****

### Results
The random guessing baseline in both cases is 50%.

Preposition-RL: most quantum models exhibit overfiting to the training set, with performance dropping close to random guessing over the OOD valid and test sets. For the classic-CLIP model, the frozen encodings are slightly worse than random on both the train and valid sets, with better performance on test. Meanwhile, the fine tuned CLIP performs best on this task, reaching 70% accuracy on the test set.

Noun-Swap: both types of quantum model performed better on the training set, however only the OHE models displayed improved validation and test performance. The fine-tuned CLIP displayed comparable accuracy, while the frozen CLIP remained near random guessing, with significant drop on the validation set. The fine-tuned CLIP test performance is worse than for the Preposition-RL task, but unclear if this is just statistical variation.

Classical-discocat: the reported results show the model reaches 99% accuracy on the training set, but 0% on the valid and test sets, suggesting extreme overfitting. This is for a task that combines Preposition-RL and Noun-Swap in some way (but it is not defined in this paper).

## Review
Overall, this seems to be an interesting piece of work, however there are issues with the clarity of the presentation - it is very difficult to figure out what is actually being evaluated for the models, as some details are missing (see suggestions below). The authors suggest that the quantum model 'outperforms classical methods' which I took to refer to the classical-discocat result, however it is unclear if the results can be directly compared as the classical-discocat model seems to have been evaluated on a different (harder?) task than the other models.
Despite this, the results are a first step towards multimodal Quantum DisCoCat, demonstrating an implementation that on one task matched the performance of classical transformer-based models.

### Typos/small things
##### Abstract
‘…semantics can successfully carry out this task~~s~~’

##### 3.1
It would be interesting to have a breakdown of which specific triples fell into which dataset (eg as an appendix). Was there any attention paid to whether both preposition labels/object orderings for a given object pair were in the OOD set?

##### 3.2.1
I think earlier, the types presented are just {n,s}, not {n,s,p} as shown here. Maybe mention the p wire in 2.1 too, or just show the simplified form directly.
'Further optimization techniques, such as rewrite functors' -> specify these, either explicitly in an appendix, or if using lambeq mention what the version you used and the name of the rewrite.
Fig 6. One of the wires has an arrowhead - I assume this is unintentional? Also I think the sphere and cylinder parametrised states should be daggered in the ansatz diagrams (order flipped and with negative angles)?

##### 3.2.2
‘each component represented by 3 qubits, resulting in an 8-bit binary encoding **for each component’**.
‘~~The structure used for representing the image vector consisted of Shape, Preposition, shape, where each took 3 qubit resulting in a 8-bit long binary encoding.~~’ redundant sentence
Fig7: are empty triangles the |0> state(/effect)? Please label them.

##### 4
Broken table 3 ref.
Wrong fig ref: Fig 2 does not display any obvious swaps. Did you mean fig 7? It might be clearer to have a separate fig where isRightOf is explicitly defined diagrammatically in terms of isLeftOf (or vice versa).
Specify how the best models were selected - since you mention two validation sets (ID and OOD) there is ambiguity as to which one (or even if a combination of both) was used.

##### 4.1
‘In general, predicting the out of distribution descriptions is a hard task since everything, **the two shapes as well as the preposition between them**, is unseen in training.’ -> surely the model has seen instances of the shapes before, just with different pairings/relationships? I think you mean ‘the OOD *triple*, (shape, preposition, shape) is unseen’.

Table 3: naming inconsistency: ‘RightvsLeft’ task -> ‘Preposition-RL’?
naming inconsistency: ‘Classic**al**-DisCoCat’ (also in table 4)

##### 4.2
naming inconsistency: TL -> Classical-DisCoCat.
naming inconsistency: Noun-Swap vs Logical-Swap
‘nearly double its previous performance’ -> misleading, since I think you mean something like ‘nearly double the distance from random guessing’? Intuitively, I’d read double to mean 110%
‘significantly small.’ Did you mean for Sim14 only? 10% in the IQP case does not seem that small to me... If you quote how wide the error bars are this might help support your statement.

### Bigger things
#### Reproducibility
There are large gaps in the description of the experiment that mean it is really difficult to figure out what circuits you actually ran, and indeed how your model actually works. I see that there are more detailed methods featured in Lewis et al (2023) - if you used the same methods from there it should be made more explicit. Either way you also need to give more complete details for the quantum model, since this is what you are introducing in this paper.
##### Circuit shapes
Figs 6 and 7 display two different ways of drawing the isLeftOf gate: which one was actually used? Also mentionned above: specify which rewrite rules were used to simplify your diagrams.
##### Getting the answer from the model
[sec 3.2] ‘… using **a** morphism of FHilb’ -> which morphism? Is it the inner product? A cup?? Maybe draw a (simplified if necessary) example of a final diagram that you evaluated, or provide a formula. This is kind of a key part of the model since its what you derive the final answer from.
Relatedly: ‘The morphism as well as the linguistic and image data are converted into a VQC whose parameters are learnt in a supervised image classification task’ As I understand it, the only parameters to be learnt are those concerning the text embedding - is this correct? It would help to state that out explicitly.
##### Embedding dimensions
The embedding dimensions are specified for the images, which is good, however there does not seem to be a reference for the text embeddings.
From reading the paper, it seems likely that the sentence type should have the same dimension as the corresponding image embedding in order to compute their inner product/overlap - if so, this should be specified.
For the quantum DisCoCat models you also need to specify how many qubits were used for the noun wires. The diagrams make this look like there's just 1 (and also just 1 qubit for the sentence wire), but this then doesn't match up with the dimensions of your image encodings.
Having a table to compare embedding sizes for each model type could be a nice way to present this.
Relatedly, the classical-DisCoCat model seems to use a CLIP image embedding with 768 dimensions, while the quantum-DisCoCat was based on 512 dimensional embeddings. Are these due to different versions of CLIP, or are both extracted by PCA from a larger dimension?
##### Amplitude encoding
‘Amplitude encoding is employed to normalize the feature vectors’ -> reference/quick description of what this means would be appreciated here.
Is the resulting state taken as a primitive, or do you model synthesising it using some standard gates/approximating it using the chosen ansatz? I assume the former, but you should make that clear.
‘ensuring their alignment with the rotational angle constraints of the quantum state space’ -> Not too sure what you mean by this? Is it just that you need to end up with a valid (normalised) quantum state?
'Rotation gates are utilized to modify the qubits’ states, enabling the storage of the image feature vectors and capturing their variations in the quantum state space' -> This makes it sound like you *are* synthesising a circuit to express the amplitude state? If so what methods do you use?
##### Dataset splits
[sec 4.1] There is mention of ID validation and test sets, but these are not defined in sec.3, nor are the results reported in the table. Please include them and mention what proportion of the train data is used for the ID validation/test sets.
For the OHE splits, it seems that all images for a certain (shape, relation, shape) triple will have the same encoding - does this not make your dataset highly redundant (such that there are effectively only 24 distinct samples in the entire set)? The reported accuracies suggest this is not the case, so I must be missing something here - where is the extra variation added?
##### Training
[sec 3.3] An explicit formula for the Classical-DisCoCirc model loss is given, but not for the quantum models actually trained in this paper. From the presentation of the dataset, I might infer that you used an analogous formula with k=1, taking the overlap of the quantum circuits with the image embedding (suggesting that the mysterious FHilb morphism is computing the inner product?).
The presentation of this section is also a bit misleading as the only training method you describe in detail is for a model that was presented in another paper.
How is the CLIP model fine-tuned? Presumably with contrastive learning like the quantum models to adjust the word embeddings? But again it's not mentioned.
How did you evaluate the quantum models? Did you simulate noise/shots or was it an exact statevector simulation?
#### Explanation/justification of choices
Some arbitrary choices could also do with some extra explanation/acknowledgement. It is expected that many choices are going to be somewhat arbitrary and constrained by the resources you had available, but it helps to mention this so it is clear that there *are* other options available.
##### OHE and embedding dimensions
[sec 3.2] Why do you use 8 bits for each component of the OHE when 4(or 2 for the prepositions) are sufficient? Also, the embeddings given for the shapes don’t look like traditional one hot encodings (the cone should be [0,0,0,1,0,0,0,0])? Alternatively, you might want to write them out as quantum states in the computational basis if that makes them clearer? Is this choice made to match the dimensions used for the text encodings? If so you should specify.
##### Noun-Swap dataset
[sec 4] 'The Logical Swap experiment is trained and tested on the same datasets as the Preposition-RL, but uses a different semantics for Prep'. -> When you say datasets, do you mean just the image-caption pairs, or the image-caption-incorrect caption triples (or even just the images)? Whether the dataset is exactly the same affects how the results are to be interpreted for the Classic-CLIP models. Since the results are different on the two tasks, I assume you mean that the pairs are the same, and have a different incorrect caption from the Preposition-RL task.

#### Evaluation
Some details are missing/would improve the provided analysis of the results:
##### Classical-DisCoCat comparison
[sec 4] It is unclear from your paper if classical-DisCoCat can really be compared to the other methods since you say it was trained/evaluated on a different version of the task, but don't present which task this is. Either remove the comparison, or explain the task and justify why you can compare them.
##### Underperformance of quantum models
[sec 4.1] ‘The observed underperformance of quantum models may stem from the inherent difficulty of differentiating spatial relationships such as “right” versus “left.”’ -> Isn’t this just saying that quantum struggled because the task is hard? If so, I don’t see a priori why the quantum model should struggle more than a classical one. Could the differences stem instead from eg a difference in the number of dimensions used in the encoding, or as you mention before, the fact that the frozen CLIP encodings perform badly. In the quantum cases, only the text encoding is trained; perhaps the the image embeddings are not sufficiently distinguishable in the first place?
##### Statistical analysis
[sec 4] Consider reporting confidence intervals/error bars for the accuracies - this will help contextualise some of the trends, and make it clearer which are robust. You should also remind what the random guessing baseline is.
##### Noun swap variants
[sec 3.2.1] Aren't the two noun-swap approaches equivalent (as witnessed by the diagram rewrites involving the swap box)? I'm not sure why distinguishing these would be important (and indeed, it seems that you didn’t train separate models for them, either).
Alternatively, if they are in fact different, you still need to provide the actual insights the different techniques provide into the workings of the model that you suggest exist.



----------------------- REVIEW 2 ---------------------
SUBMISSION: 97
TITLE: Compositional Concept Generalization with  Variational Quantum Circuits
AUTHORS: Hala Hawashin, Beth Pearson, Martha Lewis and Mehrnoosh Sadrzadeh

----------- Overall evaluation -----------
SCORE: 0 (borderline paper)
----- TEXT:
In this work, the authors present a generalization of the DiScoCat semantic model, incorporating variational quantum circuits and the FHib category to enhance the framework's performance in compositional generalization. The model is tested on text and image embeddings, with quantum circuits trained to label images (modeled as word vectors) with lexical and grammatical information.

The first part of the paper introduces the methodology and focuses on mathematical concepts, particularly categorical definitions. The authors consider two distinct categories: the (non-symmetric) grammar category generated by a pregroup and the (symmetric) meaning category of finite-dimensional real inner product spaces and linear maps.

The second (main) part of the paper presents two experiments—Preposition-RL and Logical Swap—on a dataset based on 3D geometrical shapes, comparing classical and quantum models.

I reviewed the mathematical framework, which is well-grounded in existing and established literature. The categories conform to the definition of a compact closed category and satisfy the snake equations. The examples and instances considered are clear and easy to follow.

Regarding the second part, I found the presentation somewhat confusing. For instance, important background concepts, such as notions related to image embeddings, could be introduced earlier in the methodology section rather than appearing later in the paper. In general, I suggest restructuring the paper to introduce the methodology in the first section and then describe the experiments and results in the second, avoiding back-and-forth shifts with auxiliary notions that make the reading challenging.

Focusing on the experimental results, it seems that the classical DiScoCat model outperforms other approaches. Other results seem insufficiently informative, and it is difficult to discern a clear advantage in choosing a quantum model over a classical one. This issue is particularly evident in the analysis of Experiment 2.

Overall, while the paper is interesting, it does not fully align with the scope of the QPL conference, as it lacks both significant empirical results and a clear theoretical or methodological improvement over existing techniques in Quantum NLP.

Please check the paper for typos—for example, there is a missing reference on page 10, in the first line of Section 4.



----------------------- REVIEW 3 ---------------------
SUBMISSION: 97
TITLE: Compositional Concept Generalization with  Variational Quantum Circuits
AUTHORS: Hala Hawashin, Beth Pearson, Martha Lewis and Mehrnoosh Sadrzadeh

----------- Overall evaluation -----------
SCORE: 2 (accept)
----- TEXT:
This is solid experimental towards multi-model application of quantum DisCoCat, by focussing on image labelling.  Of key interest is compositional generalisation for this task.  The results are competitive for classical training.

In recent work by Duneaux et al compositional generalisation was achieved for language, using DisCoCirc.  One may wonder if results here could be improved in that manner two.  The much-harder-to-simmulate circuits likely also give a complexity advantage assymptotically.  The fact that they are not trees makes one think that they are doing substantially more work than DisCoCat circuits.
